The Importance of Prior Knowledge in Precise Multimodal Prediction

Roads have well defined geometries, topologies, and traffic rules. While this has been widely exploited in motion planning methods to produce maneuvers that obey the law, little work has been devoted to utilize these priors in perception and motion forecasting methods. In this paper we propose to incorporate these structured priors as a loss function. In contrast to imposing hard constraints, this approach allows the model to handle non-compliant maneuvers when those happen in the real world. Safe motion planning is the end goal, and thus a probabilistic characterization of the possible future developments of the scene is key to choose the plan with the lowest expected cost. Towards this goal, we design a framework that leverages REINFORCE to incorporate non-differentiable priors over sample trajectories from a probabilistic model, thus optimizing the whole distribution. We demonstrate the effectiveness of our approach on real-world self-driving datasets containing complex road topologies and multi-agent interactions. Our motion forecasts not only exhibit better precision and map understanding, but most importantly result in safer motion plans taken by our self-driving vehicle. We emphasize that despite the importance of this evaluation, it has been often overlooked by previous perception and motion forecasting works.

==> background.tex <==
\section{Background}
To achieve safe planning, we  must effectively deal with noisy and partial observations $x$ from the sensory data, and provide an accurate characterization of the distribution of future trajectories of all actors in the scene $p(y|x)$. This is particularly challenging since the future is inherently uncertain, and actors' discrete decisions induce highly multimodal distributions (e.g turning right vs. going straight at an intersection, going vs. stopping at a yield sign).
Furthermore, datasets collected from real-world driving can only cover one possible mode out of many. As shown in  \cite{rhinehart2018r2p2}, this partial description of the underlying distribution along with a Maximum Likelihood Estimation (MLE)  objective results in high entropy distributions that favors recall over precision. In other words, though the learned distribution recovers the ground truth future, it may also generate many highly implausible samples.
\raquel{you shoudl give a high level description of what this section is going to talk about. Otherwise the reader might be surprised. We need the high level of what are you going to ttalk about, and how it relates to what you are going to propose}

While \cite{rhinehart2018r2p2} attempts to mitigate this problem by leveraging a learned characterization of the true distribution $\hat{p}(y|x)$ and a symmetrized cross entropy loss, learning this conditional prior is a very hard task since we only observe a sample from the true distribution for each input $x$ (i.e., the one that happened in reality).  An alternative is to consider leveraging prior knowledge to characterize the true distribution. In particular, the actor's motion history, road geometry, traffic rules, and nearby traffic participants all constrain the space of plausible futures.





It is difficult to represent our prior knowledge as a explicit distribution $\hat{p}(y|x)$. Instead, we can encode it as a deterministic function $r(y, x)$ of the trajectory samples from such distribution. \raquel{you need to say why this is easier.} \raquel{not clear here why the hat notation}
We can thus define a \emph{reward function} $r(y, x)$ that specifies how useful a sample from the stochastic function is for a given task. 
Then the goal  is  to learn a stochastic function (parameterized by $\theta$) that will produce the highest expected reward $r$:
\begin{align*}
J\left(\theta \right) = \mathop{\mathbb{E}_{\mathbf{y} \sim \pi_\theta\left(\mathbf{y}\right)}}\left[r\left(\mathbf{y}\right)\right]
				   = \int \pi_\theta\left(\mathbf{y}\right)r\left(\mathbf{y}\right)d\mathbf{y}
\end{align*}

Next, we discuss two common methods to optimize the expected reward over a distribution:
\raquel{give a little bit of high level about why two and why you are talking about these two}
\paragraph{Reparameterization Trick}
In the case where our prior knowledge is a differentiable reward function $r$ over the support of the distribution, and it is possible to reparameterize the sampling process \raquel{you need to talk about when its possible}, we can directly apply the loss to our samples and backpropagate the gradients as follows
\begin{align*}
& \epsilon \sim q(\epsilon), \quad y = g_{\theta}(\epsilon)\\
& \nabla J(\theta) = \nabla_{\theta}\mathbb{E}_{y\sim \pi_{\theta}(y)}[r(y)] = \mathbb{E}_{\epsilon\sim q(\epsilon)}[\nabla r(g_{\theta}(\epsilon_i)])
\end{align*}
However, these requirements are often too limiting. For instance, mixture of gaussians is a popular representation for distribution over trajectories. While each gaussian can be exactly reparameterized, it is hard to reparameterize the discrete sampling of the categorical distribution over modes. While there exist approximate reparameterizations like Gumbel-Softmax \cite{jang2016categorical}, they are biased estimators and introduce a dangerous tradeoff between how much the expectation differs from the true expected value and the ease of optimization through reparameterization (temperature hyperparameter in \cite{jang2016categorical}).
As discussed in the introduction, our intuitions about driving are not trivially transformed into a  differentiable loss function, thus requiring explicit relaxations that are biased. In Sections~\ref{pred_exp} and \ref{plan_exp} we empirically show how approximations in the relaxation can harm.

\paragraph{Policy Gradient}
In contrast, policy gradient algorithms do not assume differentiability of the reward function $r$. The most simple and popular version is the REINFORCE \cite{XX} algorithm, which  only requires the policy to be differentiable, and provides efficient sampling and likelihood evaluation. In this case, the gradient of the expected reward is estimated as:
\begin{align*}
\nabla J\left(\theta \right) = 
\mathop{\mathbb{E}_{\mathbf{y} \sim \pi_\theta\left(\mathbf{y}\right)}}
\left[\nabla \log\pi_\theta\left(\mathbf{y}\right)
r\left(\mathbf{y}\right)\right]
\end{align*}
which is generally approximated by drawing samples from the predicted distribution as follows
$$
\nabla J\left(\theta \right) \approx \frac{1}{N}\sum_i^N \sum_t^T \nabla \log\pi_\theta\left(y^i_t\right) r(y^i_t)
$$
Although this Monte Carlo estimation is unbiased, it typically has high variance. However, in our experiments we see that this does not pose a problem when using a policy that has an efficient sampling, since we can use a large number of samples $N$.









